StockGPT: A GenAI Model for Stock Prediction and Trading

This paper introduces StockGPT, an autoregressive ``number'' model trained and tested on 70 million daily U.S.\ stock returns over nearly 100 years. Treating each return series as a sequence of tokens, StockGPT automatically learns the hidden patterns predictive of future returns via its attention mechanism. On a held-out test sample from 2001 to 2023, daily and monthly rebalanced long-short portfolios formed from StockGPT predictions yield strong performance. The StockGPT-based portfolios span momentum and long-/short-term reversals, eliminating the need for manually crafted price-based strategies, and yield highly significant alphas against leading stock market factors, suggesting a novel AI pricing effect. This highlights the immense promise of generative AI in surpassing human in making complex financial investment decisions.

==> tables/Daily_NYSE_Spanning_Others_Alpha_Slides.tex <==

  \providecommand{\huxb}[2]{\arrayrulecolor[RGB]{#1}\global\arrayrulewidth=#2pt}
  \providecommand{\huxvb}[2]{\color[RGB]{#1}\vrule width #2pt}
  \providecommand{\huxtpad}[1]{\rule{0pt}{#1}}
  \providecommand{\huxbpad}[1]{\rule[-#1]{0pt}{#1}}
\begin{tabular}{l l l l l l l l l l l l l}


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt}  \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt}  \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} ST\_Rev \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} Mom \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} LT\_Rev \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} MKT \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} HML \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} SMB \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} RMW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} CMA \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_IA \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_ROE \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_EG \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\alpha$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -40.19 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 9.23 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.33 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -25.98 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.89 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.90 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 10.20 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 6.72 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 6.68 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 9.37 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 8.85 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\alpha}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -6.11 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.57 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.44 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -3.47 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.18 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 4.30 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.66 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.27 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.71 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\beta$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.42 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.06 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.29 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.03 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\beta}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 9.19 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.92 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.13 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 7.51 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.59 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.39 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -4.75 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -4.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -3.50 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -3.59 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.82 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $R^2$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 25.69 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.45 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.66 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 7.28 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.27 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.27 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.09 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.96 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.60 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\alpha$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.17 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.96 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.21 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.30 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.74 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 4.50 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.61 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.38 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.45 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.10 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\alpha}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.75 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.48 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.52 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.28 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.46 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.46 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.66 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.39 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.52 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.64 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\beta$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.27 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.00 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.12 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.01 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.00 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.01 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.00 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\beta}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 8.18 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.14 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.50 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.32 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.53 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.51 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.12 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.99 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.65 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.99 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.28 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $R^2$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 22.82 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.01 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.95 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.38 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.28 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.85 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.65 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.12 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.00 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}-}
\arrayrulecolor{black}
\end{tabular}

==> tables/Monthly_Ret20_NYSE_Spanning_Others_Alpha_Slides.tex <==

  \providecommand{\huxb}[2]{\arrayrulecolor[RGB]{#1}\global\arrayrulewidth=#2pt}
  \providecommand{\huxvb}[2]{\color[RGB]{#1}\vrule width #2pt}
  \providecommand{\huxtpad}[1]{\rule{0pt}{#1}}
  \providecommand{\huxbpad}[1]{\rule[-#1]{0pt}{#1}}
\begin{tabular}{l l l l l l l l l l l l l}


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt}  \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt}  \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} ST\_Rev \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} Mom \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} LT\_Rev \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} MKT \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} HML \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} SMB \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} RMW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} CMA \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_IA \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_ROE \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} R\_EG \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\alpha$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 9.00 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.83 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.33 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 6.15 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.14 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.35 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 6.06 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.84 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.44 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.69 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\alpha}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 4.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.98 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.97 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.65 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.74 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.91 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.10 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.50 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.11 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.77 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.95 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\beta$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.14 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.10 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.07 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.08 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.08 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.02 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.09 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.03 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\beta}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.21 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.60 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.78 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.40 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.39 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.77 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.33 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.99 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.46 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} EW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $R^2$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.33 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.46 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.53 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.43 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.34 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.08 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.36 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.26 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.28 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.17 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}->{\huxb{0, 0, 0}{0.8}}-}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\alpha$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 9.27 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.77 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.13 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 7.85 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.18 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.42 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 5.00 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.77 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.34 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 3.70 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 4.72 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\alpha}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 4.34 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.52 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.94 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.17 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.80 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.92 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.67 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.60 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.25 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 0}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.68 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\cellcolor[RGB]{255, 255, 255}\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.26 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $\beta$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.14 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.08 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.10 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.01 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.04 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.03 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.05 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.05 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $t_{\beta}$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.68 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.48 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -3.55 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.40 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.50 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -2.69 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.21 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -1.30 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.78 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.90 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.24 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{}
\arrayrulecolor{black}

\multicolumn{1}{!{\huxvb{0, 0, 0}{0}}l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} VW \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{l!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedright \hspace{0pt} $R^2$ \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.29 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.23 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 10.92 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.16 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.85 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 6.68 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} -0.31 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.69 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 0.35 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 1.19 \hspace{0pt}\huxbpad{0pt}} &
\multicolumn{1}{r!{\huxvb{0, 0, 0}{0}}}{\huxtpad{0pt + 1em}\raggedleft \hspace{0pt} 2.15 \hspace{0pt}\huxbpad{0pt}} \tabularnewline[-0.5pt]


\hhline{>{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}->{\huxb{0, 0, 0}{0.6}}-}
\arrayrulecolor{black}
\end{tabular}
